Calibration of the AdvancedVirgo+ Gravitational Wave Detector and Reconstruction of the Detector Strain h(t) during the Observing Run O4

From 10 April 2024 15:00 UTC to 18 November 2025 16:00 UTC, the AdvancedVirgo+ gravitational wave detector participated in the LIGO-Virgo-KAGRA O4 observing run, started on 24 May 2023 15:00 UTC. Around 173 transient gravitational wave (GW) sources, all corresponding to coalescences of binary compact objects involving black holes and neutron stars, were detected online during the two run periods O4b and O4c when Virgo was taking data in the detector network. Despite its sensitivity being limited around 55 Mpc, the inclusion of Virgo into the network allowed to improve the accuracy of the source parameter estimation, in particular the sky localisation of the detected events. This article describes the AdvancedVirgo+ detector calibration and the reconstruction of the detector strain h(t) during O4, as well as the estimation of the associated frequency-dependent uncertainties. The detector calibration is based on auxiliary actuators, Newtonian Calibrators and Photon Calibrators, described in other publications. The h(t) reconstruction, including linear noise subtraction, was processed online with a latency of about 10 s. The so-called AnalysisReady strain data were then produced offline. Most of the time, the strain time series was a copy of the online time series, but with updated frequency-dependent uncertainties, around 2-3% in amplitude and below 30 mrad in phase in the 10-2000 Hz frequency band, with the exception of larger uncertainties around 50 Hz and 150 Hz. The AnalysisReady strain data and associated uncertainties have been used for the offline LIGO-Virgo-KAGRA data analysis and are also the data made publicly available through the Gravitational Wave Open Science Center (GWOSC).

==> definitions.tex <==

\RequirePackage{xspace}

\newcommand{\dv}[1]{{\color{magenta} #1}}
\newcommand{\lr}[1]{{\color{blue} #1}}
\newcommand{\msa}[1]{{\color{orange} #1}}
\newcommand{\cg}[1]{{\color{red} #1}}
%
\newcommand{\de}[1]{{\color{darkgreen} Dimitri: #1}}
\newcommand{\paul}[1]{{\color{cyan} Paul: #1}}
\newcommand{\todo}[1]{{\color{red} TO-DO: #1}}
\newcommand*\rot{\rotatebox{90}} 

\newcommand{\dg}{\ensuremath{^\circ}}
\newcommand{\VIRGO}{\small VIRGO}
\newcommand{\AdV}{\small AdvancedVirgo+}
\newcommand{\RMS}{{\small RMS}}
\newcommand{\RMSs}{{\small RMS}s}
\newcommand{\ADC}{{\small ADC}}
\newcommand{\ADCs}{{\small ADC}s}
\newcommand{\DAC}{{\small DAC}}
\newcommand{\DACs}{{\small DAC}s}
\newcommand{\GW}{GW}
\newcommand{\GWs}{GWs}
\newcommand{\ITF}{ITF}
\newcommand{\TF}{TF}
\newcommand{\TFs}{TFs}
\newcommand{\FFT}{FFT}
\newcommand{\FFTs}{FFTs}
\newcommand{\HP}{HP}
\newcommand{\LN}{LN}
\newcommand{\DSP}{DSP}
\newcommand{\DSPs}{DSPs}
\newcommand{\NE}{NE}
\newcommand{\NI}{NI}
\newcommand{\WE}{WE}
\newcommand{\WI}{WI}
\newcommand{\BS}{BS}
%\newcommand{\PR}{PR}
\newcommand{\TEMOO}{$\mathrm{TEM_{00}}$}
\newcommand{\mus}  {$\upmu \text{s}$}
\newcommand{\mum}  {$\upmu \text{m}$}
\newcommand{\murad}{$\upmu \text{rad}$}

\newcommand{\PrBACp}{$\mathrm{Pr\_B1\_ACp}$}
\newcommand{\prl}{Phys. Rev. Letters}
\newcommand{\SczCorr}{$\mathrm{Sc\_*\_zCorr}$}
\newcommand\rednote[1]{\textcolor{red}{\bf {#1}}}
\newcommand\bluenote[1]{\textcolor{blue}{\bf {#1}}}

\newcommand{\VirgoAcronym}[3]{ \noindent {\bf #1}: {\it #2}, #3. \\}
\newcommand{\VirgoAcronymShort}[2]{ \noindent {\bf #1}: #2. \\}

